Finite Quotients of Right-angled Artin Groups

We prove that right-angled Artin groups (RAAGs) are profinitely rigid relative to the class of Artin groups. More precisely, if $A_\Gamma$ is an arbitrary Artin group and $A_\Lambda$ is a right-angled Artin group such that their profinite completions are isomorphic, i.e., $\widehat{A_\Gamma}\cong\widehat{A_\Lambda},$ then $\Gamma$ is right-angled and $\Gamma\cong\Lambda$ as labeled graphs. The proof combines the structure of pro-$p$ completions of Artin groups with finite Coxeter quotients to recover the defining graph.

==> references.bib.tex <==
@article{Droms87,
    author  = {Droms, Carl},
    title   = {Isomorphisms of Graph Groups},
    journal = {Proceedings of the American Mathematical Society},
    volume  = {100},
    number  = {3},
    year    = {1987},
    pages   = {407--408},
    doi     = {10.1090/S0002-9939-1987-0891135-8}
}

@article{KW16,
    author  = {Kropholler, Robert and Wilkes, Gareth},
    title   = {Profinite Properties of {RAAG}s and Special Groups},
    journal = {Bulletin of the London Mathematical Society},
    volume  = {48},
    number  = {6},
    year    = {2016},
    pages   = {1001--1007},
    doi     = {10.1112/blms/bdw056}
}

@article{CPZ25,
    author  = {Casals-Ruiz, Montserrat and Pintonello, Matteo and
               Zalesskii, Pavel},
    title   = {Pro-$\mathcal{C}$ {RAAG}s},
    journal = {Journal of Algebra},
    volume  = {664},
    year    = {2025},
    pages   = {177--208},
    doi     = {10.1016/j.jalgebra.2024.09.030}
}

@misc{ELMP26,
    author        = {Escart{\'i}n Ferrer, Marcos and Leoni, Giorgio and
                     Mart{\'i}nez P{\'e}rez, Conchita},
    title         = {Cohomology Rings and $p$-Local Behavior of Even
                     {Artin} Groups},
    year          = {2026},
    eprint         = {2606.30558},
    archivePrefix = {arXiv},
    primaryClass  = {math.GR},
    note          = {arXiv:2606.30558v1}
}

@article{Mol18,
    author  = {Moldavanskii, David I.},
    title   = {On the Residual Properties of {Baumslag--Solitar}
               Groups},
    journal = {Communications in Algebra},
    volume  = {46},
    number  = {9},
    year    = {2018},
    pages   = {3766--3778},
    doi     = {10.1080/00927872.2018.1424867}
}

@book{Dav08,
    author    = {Davis, Michael W.},
    title     = {The Geometry and Topology of Coxeter Groups},
    series    = {London Mathematical Society Monographs Series},
    volume    = {32},
    publisher = {Princeton University Press},
    address   = {Princeton, NJ},
    year      = {2008},
    isbn      = {978-0-691-13138-2}
}


